The Illusion of Fit: Spatially Resolved Assessment of Constitutive Model Validity in Elastography and Physics-Based Inverse Problems

Inferring the mechanical properties of soft tissues from measured deformations is a fundamental challenge in elastography. A rarely examined assumption underlying existing approaches is that the assumed constitutive law correctly describes the imaged material. When it fails, inversion still yields plausible-looking estimates - an illusion of fit with no indication of local model invalidity, which can mislead clinical interpretation. We propose a probabilistic framework that transforms constitutive model validity from an implicit assumption into an explicit, spatially resolved inference target. The key is to treat the stress field as an independent latent variable rather than deriving it from the constitutive law. This enables a pointwise comparison between the stress required by mechanical equilibrium and the stress predicted by the assumed constitutive model. Both governing equations enter the probabilistic learning objective as virtual observables with separate precision hyperparameters: the conservation law precision is set a priori to a small value reflecting its undisputed validity, while the constitutive precision is inferred under a sparsity-promoting prior. The resulting constitutive precision field provides an uncertainty-aware map of where the assumed model is supported by the data and where it is not. Inference is carried out via stochastic variational inference and is forward-model-free. We validate the framework on synthetic harmonic elastography experiments on a brain-slice geometry with an anisotropic inclusion. The inferred precision field identifies the inclusion with a five-order-of-magnitude precision contrast against the valid domain, robustly across 25-35 dB noise and four-fold sparser observations. A phantom experiment with ultrasound measurements on a linear elastic material yields no false-positive violations and recovers the true stiffness contrast.

==> Sections/definitions_doc.tex <==
%\usepackage{hyperref}
\usepackage[normalem]{ulem}


\usepackage{setspace}
\usepackage{comment}
\usepackage{amsmath,amsthm,amssymb}
\usepackage{ulem}
%\renewcommand{\baselinestretch}{1.4}

\newcommand{\bs}{\boldsymbol}
\def\RR{ \mathbb R}
\newcommand{\refeqp}[1]{Equation (\ref{#1})}
\def\bl{ \mathbf \lambda}
\def\ba{ \beta}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\boxeq}[1]{%
  \[\fbox{%
      \addtolength{\linewidth}{-2\fboxsep}%
      \addtolength{\linewidth}{-2\fboxrule}%
      \begin{minipage}{\linewidth}%
      \begin{equation}#1\end{equation}%
      \end{minipage}%
    }\]%
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\ee}{\end{equation}}
\newcommand{\be}{\begin{equation}}
\newcommand{\ec}{\end{center}}
\newcommand{\bc}{\begin{center}}
\newcommand{\eea}{\end{eqnarray}}
\newcommand{\bea}{\begin{eqnarray}}
\newcommand{\bd}{\begin{description}}
\newcommand{\ed}{\end{description}}
\newcommand{\bi}{\begin{itemize}}
\newcommand{\ei}{\end{itemize}}
\newcommand{\pa}{\partial}
\newcommand\bphi{\boldsymbol{\phi}}
\newcommand\bpsi{\boldsymbol{\psi}}

\newcommand{\bx}{\bs{x}}
\newcommand{\bxi}{\bx^{(i)}}
\newcommand{\bxn}{\bx^{(n)}}

\newcommand{\by}{\bs{y}}
\newcommand{\byn}{\by^{(n)}}

\newcommand{\br}{\bs{r}} 
\newcommand{\brn}{\bs{r}^{(n)}} 

\newcommand{\bz}{\bs{z}}



\newcommand{\bxx}{\bs{X}}
\newcommand{\bxb}{\bar{\bs{X}}}
\newcommand{\byy}{\bs{Y}}

\newcommand{\bt}{\bs{\theta}}
\newcommand{\btt}{\bs{\Theta}}


\newcommand{\bp}{\bs{\phi}}
\newcommand{\bps}{\bs{\psi}}


\newcommand{\beps}{\bs{\epsilon}}
\newcommand{\qe}{q_{\epsilon}(\bs{\epsilon})}

\newcommand{\bax}{\bs{A}_x}
\newcommand{\bbx}{\bs{b}_x}
\newcommand{\bvx}{\bs{V}_x}
\newcommand{\bcx}{\bs{C}_x}
\newcommand{\bdx}{\bs{D}_x}
%%%%%%%%%%%%%%%%%%%%%yaohua's newcommand
\newcommand{\Ncal}{\mathcal{N}}
% \newcommand{\Ical}{\mathcal{I}}
\newcommand{\Bcal}{\mathcal{B}}
\newcommand{\Acal}{\mathcal{A}}
\newcommand{\Dcal}{\mathcal{D}}
\newcommand{\Ecal}{\mathcal{E}}
\newcommand{\Ucal}{\mathcal{U}}
\newcommand{\Rbb}{\mathbb{R}}
\newcommand{\Gcal}{\mathcal{G}}
\newcommand{\Lcal}{\mathcal{L}}
\newcommand{\Hcal}{\mathcal{H}}
\newcommand{\Mcal}{\mathcal{M}}
\newcommand{\Rcal}{\mathcal{R}}
%
\newcommand{\bmx}{\bm{x}}
\newcommand{\bmbeta}{\bm{\beta}}

\newenvironment{colbox}[1]{        % Riddle environment
  \begin{center}                   % Centering minipage
    \colorbox[HTML]{F8E0E0} {          % Set's the color of minipage
      \begin{minipage}[b]{380px}   % Starts minipage
   \textbf{Research Question:}\\ \textit{#1}       % Set's title and starts italic for text
  \end{minipage} }                 % End minipage
}{\end{center}}
%--------------------------------------------------

%\usepackage{amsmath,amsthm,amssymb}
\usepackage{commath}
\usepackage{mathtools}
\usepackage{algorithm,algorithmic}
\usepackage{hyperref}
\usepackage{color}
\usepackage{amsfonts}

\usepackage{diagbox}
\usepackage{bm}
\usepackage{booktabs}       % professional-quality tables
%\usepackage{appendix}
\usepackage{multirow}
%
%\usepackage{graphicx}
\usepackage{subfigure}
\usepackage[percent]{overpic}
\usepackage{caption}

\newtheorem{theorem}{Theorem}
%\DeclareMathOperator*{\argmin}{\mathrm{arg\,min}}
%\DeclareMathOperator*{\argmax}{\mathrm{arg\,max}}

%
\newcommand{\zang}[1]{\textcolor{blue}{zang: #1}}
\newcommand{\psk}[1]{\textcolor{red}{PSK: #1}}
%
\newcommand{\bmm}{{\bm{m}}}
\newcommand{\bmphi}{{\bm{\varphi}}}
\newcommand{\bmz}{{\bm{z}}}
\newcommand{\bmza}{{\bm{z}_0}}
\newcommand{\bmzb}{{\bm{z}_1}}
\newcommand{\bmtheta}{{\bm{\theta}}}
\newcommand{\bmeta}{{\bm{\eta}}}
\newcommand{\bmxi}{{\bm{\xi}}}
%
\newcommand{\Rhat}{{\hat{R}}}
\newcommand{\bmRhat}{{\bm{\hat{R}}}}
%%%%
\algnewcommand{\Inputs}[1]{%
  \State \textbf{Inputs:}
  \Statex \hspace*{\algorithmicindent}\parbox[t]{.8\linewidth}{\raggedright #1}
}
\algnewcommand{\Initialize}[1]{%
  \State \textbf{Initialize:}
  \Statex \hspace*{\algorithmicindent}\parbox[t]{.8\linewidth}{\raggedright #1}
}
\algnewcommand{\Outputs}[1]{%
  \State \textbf{Outputs:}
  \Statex \hspace*{\algorithmicindent}\parbox[t]{.8\linewidth}{\raggedright #1}
}

